A boundary-oriented reduced Schwarz domain decomposition technique for parametric advection-diffusion problems

We present in this paper the results of a research motivated by the need of a very fast solution of thermal flow in solar receivers. These receivers are composed by a large number of parallel pipes with the same geometry. We have introduced a reduced Schwarz algorithm that skips the computation in a large part of the pipes. The computation of the temperature in the skep domain is replaced by a reduced mapping that provides the transmission conditions. This reduced mapping is computed in an off-line stage. We have performed an error analysis of the reduced Schwarz algorithm, proving that the error is bounded in terms of the linearly decreasing error of the standard Schwarz algorithm, plus the error stemming from the reduction of the trace mapping. The last error is asymptotically dominant in the Schwarz iterative process. We obtain $L^2$ errors below $2\%$ with relatively small overlapping lengths.

==> Biblio.tex <==
@article {MR4563153,
    AUTHOR = {Li, Kun and Huang, Ting-Zhu and Li, Liang and Lanteri,
              St\'{e}phane},
     TITLE = {Simulation of the interaction of light with 3-{D} metallic
              nanostructures using a proper orthogonal
              decomposition-{G}alerkin reduced-order discontinuous
              {G}alerkin time-domain method},
   JOURNAL = {Numer. Methods Partial Differential Equations},
  FJOURNAL = {Numerical Methods for Partial Differential Equations. An
              International Journal},
    VOLUME = {39},
      YEAR = {2023},
    NUMBER = {2},
     PAGES = {932--954},
      ISSN = {0749-159X},
   MRCLASS = {65M60 (65F25 78A45 78M10)},
  MRNUMBER = {4563153},
}
		
@article {MR4106667,
    AUTHOR = {Reyes, Ricardo and Codina, Ramon},
     TITLE = {Element boundary terms in reduced order models for flow
              problems: domain decomposition and adaptive coarse mesh
              hyper-reduction},
   JOURNAL = {Comput. Methods Appl. Mech. Engrg.},
  FJOURNAL = {Computer Methods in Applied Mechanics and Engineering},
    VOLUME = {368},
      YEAR = {2020},
     PAGES = {113159, 27},
      ISSN = {0045-7825},
   MRCLASS = {65M60 (65M15 65M50 65M55)},
  MRNUMBER = {4106667},
       DOI = {10.1016/j.cma.2020.113159},
       URL = {https://doi.org/10.1016/j.cma.2020.113159},
}
		
@article {MR3959737,
    AUTHOR = {Xiao, D. and Fang, F. and Heaney, C. E. and Navon, I. M. and
              Pain, C. C.},
     TITLE = {A domain decomposition method for the non-intrusive reduced
              order modelling of fluid flow},
   JOURNAL = {Comput. Methods Appl. Mech. Engrg.},
  FJOURNAL = {Computer Methods in Applied Mechanics and Engineering},
    VOLUME = {354},
      YEAR = {2019},
     PAGES = {307--330},
      ISSN = {0045-7825},
   MRCLASS = {65M60 (65M55 76D05 76M10)},
  MRNUMBER = {3959737},
       DOI = {10.1016/j.cma.2019.05.039},
       URL = {https://doi.org/10.1016/j.cma.2019.05.039},
}
		
@article {MR3916891,
    AUTHOR = {Xiao, D. and Heaney, C. E. and Fang, F. and Mottet, L. and Hu,
              R. and Bistrian, D. A. and Aristodemou, E. and Navon, I. M.
              and Pain, C. C.},
     TITLE = {A domain decomposition non-intrusive reduced order model for
              turbulent flows},
   JOURNAL = {Comput. \& Fluids},
  FJOURNAL = {Computers \& Fluids. An International Journal},
    VOLUME = {182},
      YEAR = {2019},
     PAGES = {15--27},
      ISSN = {0045-7930},
   MRCLASS = {65M60 (76D05 76M10)},
  MRNUMBER = {3916891},
       DOI = {10.1016/j.compfluid.2019.02.012},
       URL = {https://doi.org/10.1016/j.compfluid.2019.02.012},
}
		
@article {MR3807827,
    AUTHOR = {Stefanescu, Razvan and Moosavi, Azam and Sandu, Adrian},
     TITLE = {Parametric domain decomposition for accurate reduced order
              models: applications of {MP}-{LROM} methodology},
   JOURNAL = {J. Comput. Appl. Math.},
  FJOURNAL = {Journal of Computational and Applied Mathematics},
    VOLUME = {340},
      YEAR = {2018},
     PAGES = {629--644},
      ISSN = {0377-0427},
   MRCLASS = {65M99},
  MRNUMBER = {3807827},
       DOI = {10.1016/j.cam.2017.11.018},
       URL = {https://doi.org/10.1016/j.cam.2017.11.018},
}
		
@article {MR3127293,
    AUTHOR = {Baiges, Joan and Codina, Ramon and Idelsohn, Sergio},
     TITLE = {A domain decomposition strategy for reduced order models.
              {A}pplication to the incompressible {N}avier-{S}tokes
              equations},
   JOURNAL = {Comput. Methods Appl. Mech. Engrg.},
  FJOURNAL = {Computer Methods in Applied Mechanics and Engineering},
    VOLUME = {267},
      YEAR = {2013},
     PAGES = {23--42},
      ISSN = {0045-7825},
   MRCLASS = {65N30 (76D05)},
  MRNUMBER = {3127293},
       DOI = {10.1016/j.cma.2013.08.001},
       URL = {https://doi.org/10.1016/j.cma.2013.08.001},
}

@article {MR4538344,
    AUTHOR = {Gander, Martin J. and Lunowa, Stephan B. and Rohde, Christian},
     TITLE = {Non-overlapping {S}chwarz waveform-relaxation for nonlinear
              advection-diffusion equations},
   JOURNAL = {SIAM J. Sci. Comput.},
  FJOURNAL = {SIAM Journal on Scientific Computing},
    VOLUME = {45},
      YEAR = {2023},
    NUMBER = {1},
     PAGES = {A49--A73},
      ISSN = {1064-8275},
   MRCLASS = {65M55 (35K55 35L65 76S05)},
  MRNUMBER = {4538344},
       DOI = {10.1137/21M1415005},
       URL = {https://doi.org/10.1137/21M1415005},
}
		
@article {MR4506712,
    AUTHOR = {Lorin, Emmanuel and Yang, Xu},
     TITLE = {Schwarz waveform relaxation-learning for
              advection-diffusion-reaction equations},
   JOURNAL = {J. Comput. Phys.},
  FJOURNAL = {Journal of Computational Physics},
    VOLUME = {473},
      YEAR = {2023},
     PAGES = {Paper No. 111657, 16},
      ISSN = {0021-9991},
   MRCLASS = {65M55 (68T07)},
  MRNUMBER = {4506712},
MRREVIEWER = {Tao Liu},
       DOI = {10.1016/j.jcp.2022.111657},
       URL = {https://doi.org/10.1016/j.jcp.2022.111657},
}
		
@incollection {MR3977048,
    AUTHOR = {Gander, Martin J. and Vanzan, Tommaso},
     TITLE = {Optimized {S}chwarz methods for advection diffusion equations
              in bounded domains},
 BOOKTITLE = {Numerical mathematics and advanced applications---{ENUMATH}
              2017},
    SERIES = {Lect. Notes Comput. Sci. Eng.},
    VOLUME = {126},
     PAGES = {921--929},
 PUBLISHER = {Springer, Cham},
      YEAR = {2019},
   MRCLASS = {65N55},
  MRNUMBER = {3977048},
       DOI = {10.1007/978-3-319-96415-7\_87},
       URL = {https://doi.org/10.1007/978-3-319-96415-7_87},
}
		
@article {MR3845924,
    AUTHOR = {Boulaaras, Salah and Touati Brahim, Mohammed Said and
              Bouzenada, Smail},
     TITLE = {A posteriori error estimates for the generalized {S}chwarz
              method of a new class of advection-diffusion equation with
              mixed boundary condition},
   JOURNAL = {Math. Methods Appl. Sci.},
  FJOURNAL = {Mathematical Methods in the Applied Sciences},
    VOLUME = {41},
      YEAR = {2018},
    NUMBER = {14},
     PAGES = {5493--5505},
      ISSN = {0170-4214},
   MRCLASS = {65M60 (65M15)},
  MRNUMBER = {3845924},
       DOI = {10.1002/mma.5092},
       URL = {https://doi.org/10.1002/mma.5092},
}
		
@book {MR3828641,
    AUTHOR = {Chakravarty, Lopamudra},
     TITLE = {Scalable {H}ybrid {S}chwarz {D}omain {D}ecomposition
              {A}lgorithms to {S}olve {A}dvection-{D}iffusion {P}roblems},
      NOTE = {Thesis (Ph.D.)--Kent State University},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2018},
     PAGES = {132},
      ISBN = {978-0438-07173-5},
   MRCLASS = {Thesis},
  MRNUMBER = {3828641},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:10868375},
}
		
@article {MR3555348,
    AUTHOR = {Bennequin, Daniel and Gander, Martin J. and Gouarin, Loic and
              Halpern, Laurence},
     TITLE = {Optimized {S}chwarz waveform relaxation for advection reaction
              diffusion equations in two dimensions},
   JOURNAL = {Numer. Math.},
  FJOURNAL = {Numerische Mathematik},
    VOLUME = {134},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {513--567},
      ISSN = {0029-599X},
   MRCLASS = {65M60 (65M15 65M55)},
  MRNUMBER = {3555348},
MRREVIEWER = {Mohammad Asadzadeh},
       DOI = {10.1007/s00211-015-0784-8},
       URL = {https://doi.org/10.1007/s00211-015-0784-8},
}
		
@incollection {MR3645193,
    AUTHOR = {Halpern, Laurence and Hubert, Florence},
     TITLE = {A finite volume {V}entcell-{S}chwarz algorithm for
              advection-diffusion equations},
 BOOKTITLE = {Domain decomposition methods in science and engineering {XXI}},
    SERIES = {Lect. Notes Comput. Sci. Eng.},
    VOLUME = {98},
     PAGES = {937--946},
 PUBLISHER = {Springer, Cham},
      YEAR = {2014},
   MRCLASS = {65N08 (65N55)},
  MRNUMBER = {3645193},
}
		
@article {MR3213798,
    AUTHOR = {Halpern, Laurence and Hubert, Florence},
     TITLE = {A finite volume {V}entcell-{S}chwarz algorithm for
              advection-diffusion equations},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {52},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {1269--1291},
      ISSN = {0036-1429},
   MRCLASS = {65N08 (65N55)},
  MRNUMBER = {3213798},
MRREVIEWER = {Srinivasan Natesan},
       DOI = {10.1137/130919799},
       URL = {https://doi.org/10.1137/130919799},
}
		
@article {MR2566080,
    AUTHOR = {Nourtier-Mazauric, Elise and Blayo, Eric},
     TITLE = {Towards efficient interface conditions for a {S}chwarz domain
              decomposition algorithm for an advection equation with
              biharmonic diffusion},
   JOURNAL = {Appl. Numer. Math.},
  FJOURNAL = {Applied Numerical Mathematics. An IMACS Journal},
    VOLUME = {60},
      YEAR = {2010},
    NUMBER = {1-2},
     PAGES = {83--93},
      ISSN = {0168-9274},
   MRCLASS = {65M55 (35J40 35K57 65M60)},
  MRNUMBER = {2566080},
MRREVIEWER = {Beny Neta},
       DOI = {10.1016/j.apnum.2009.10.001},
       URL = {https://doi.org/10.1016/j.apnum.2009.10.001},
}
		
@article {MR2512560,
    AUTHOR = {Daoud, Daoud S. and Gander, Martin J.},
     TITLE = {Overlapping {S}chwarz waveform relaxation for advection
              reaction diffusion equations},
   JOURNAL = {Bol. Soc. Esp. Mat. Apl. SeMA},
  FJOURNAL = {Bolet\'{\i}n de la Sociedad Espa\~{n}ola de Matem\'{a}tica Aplicada. SeMA},
    NUMBER = {46},
      YEAR = {2009},
     PAGES = {75--90},
      ISSN = {1575-9822},
   MRCLASS = {65M12 (35K20 35K57)},
  MRNUMBER = {2512560},
MRREVIEWER = {Ricardo Ruiz Baier},
}
		
@book {MR2711738,
    AUTHOR = {Dubois, Olivier},
     TITLE = {Optimized {S}chwarz methods for the advection-diffusion
              equation and for problems with discontinuous coefficients},
      NOTE = {Thesis (Ph.D.)--McGill University (Canada)},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2007},
     PAGES = {209},
      ISBN = {978-0494-38582-1},
   MRCLASS = {Thesis},
  MRNUMBER = {2711738},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:NR38582},
}
		
@incollection {MR2334114,
    AUTHOR = {Gander, Martin J. and Halpern, Laurence and Kern, Michel},
     TITLE = {A {S}chwarz waveform relaxation method for
              advection-diffusion-reaction problems with discontinuous
              coefficients and non-matching grids},
 BOOKTITLE = {Domain decomposition methods in science and engineering {XVI}},
    SERIES = {Lect. Notes Comput. Sci. Eng.},
    VOLUME = {55},
     PAGES = {283--290},
 PUBLISHER = {Springer, Berlin},
      YEAR = {2007},
   MRCLASS = {65M55},
  MRNUMBER = {2334114},
       DOI = {10.1007/978-3-540-34469-8\_33},
       URL = {https://doi.org/10.1007/978-3-540-34469-8_33},
}
		
@incollection {MR2334102,
    AUTHOR = {Dubois, Olivier},
     TITLE = {Optimized {S}chwarz methods with {R}obin conditions for the
              advection-diffusion equation},
 BOOKTITLE = {Domain decomposition methods in science and engineering {XVI}},
    SERIES = {Lect. Notes Comput. Sci. Eng.},
    VOLUME = {55},
     PAGES = {181--188},
 PUBLISHER = {Springer, Berlin},
      YEAR = {2007},
   MRCLASS = {65N55},
  MRNUMBER = {2334102},
MRREVIEWER = {Renato G. C. Spigler},
       DOI = {10.1007/978-3-540-34469-8\_18},
       URL = {https://doi.org/10.1007/978-3-540-34469-8_18},
}
		
@article {MR2300292,
    AUTHOR = {Gander, M. J. and Halpern, L.},
     TITLE = {Optimized {S}chwarz waveform relaxation methods for advection
              reaction diffusion problems},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {45},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {666--697},
      ISSN = {0036-1429},
   MRCLASS = {65M55 (65M70)},
  MRNUMBER = {2300292},
MRREVIEWER = {Michael Fr\"{o}hner},
       DOI = {10.1137/050642137},
       URL = {https://doi.org/10.1137/050642137},
}
		
@article {MR1627223,
    AUTHOR = {Mathew, T. P.},
     TITLE = {Uniform convergence of the {S}chwarz alternating method for
              solving singularly perturbed advection-diffusion equations},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {35},
      YEAR = {1998},
    NUMBER = {4},
     PAGES = {1663--1683},
      ISSN = {0036-1429},
   MRCLASS = {65N12},
  MRNUMBER = {1627223},
MRREVIEWER = {Martin Stynes},
       DOI = {10.1137/S0036142995296485},
       URL = {https://doi.org/10.1137/S0036142995296485},
}
		
@article {MR1484319,
    AUTHOR = {Brakkee, Erik and Wilders, Peter},
     TITLE = {The influence of interface conditions on convergence of
              {K}rylov-{S}chwarz domain decomposition for the
              advection-diffusion equation},
   JOURNAL = {J. Sci. Comput.},
  FJOURNAL = {Journal of Scientific Computing},
    VOLUME = {12},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {11--30},
      ISSN = {0885-7474},
   MRCLASS = {65M55},
  MRNUMBER = {1484319},
MRREVIEWER = {Tsorng-Whay Pan},
       DOI = {10.1023/A:1025602319278},
       URL = {https://doi.org/10.1023/A:1025602319278},
}
